Review4Repair: Code Review Aided Automatic Program Repairing

Context: Learning-based automatic program repair techniques are showing promise to provide quality fix suggestions for detected bugs in the source code of the software. These tools mostly exploit historical data of buggy and fixed code changes and are heavily dependent on bug localizers while applying to a new piece of code. With the increasing popularity of code review, dependency on bug localizers can be reduced. Besides, the code review-based bug localization is more trustworthy since reviewers' expertise and experience are reflected in these suggestions. Objective: The natural language instructions scripted on the review comments are enormous sources of information about the bug's nature and expected solutions. However, none of the learning-based tools has utilized the review comments to fix programming bugs to the best of our knowledge. In this study, we investigate the performance improvement of repair techniques using code review comments. Method: We train a sequence-to-sequence model on 55,060 code reviews and associated code changes. We also introduce new tokenization and preprocessing approaches that help to achieve significant improvement over state-of-the-art learning-based repair techniques. Results: We boost the top-1 accuracy by 20.33% and top-10 accuracy by 34.82%. We could provide a suggestion for stylistics and non-code errors unaddressed by prior techniques. Conclusion: We believe that the automatic fix suggestions along with code review generated by our approach would help developers address the review comment quickly and correctly and thus save their time and effort.

==> Sections/Approach.tex <==






==> Sections/Background.tex <==
This section presents a brief background on models and terminology relevant to this research.

\textbf{Sequence-to-Sequence Model:} Sequence-to-sequence (seq2seq) models are a class of machine learning techniques that transfers a sequence to another sequence~\cite{seq2seq}. Seq2seq models consist of two parts: encoder and decoder. The encoder converts a sequence of input tokens to a hidden representation, and the decoder produces the desired sequence from that hidden representation. Commonly seq2seq models use Recurrent Neural Networks (RNN) or one of its variants, LSTM~\cite{hochreiter1997long} or GRU~\cite{gru}. The seq2seq model is agnostic of the nature of the sequence. Therefore, the same seq2seq approach that is used to translate the natural language (e.g., English and French) has been found effective to translate from a buggy code to a correct code \cite{tufano2019learning, chen2018sequencer, codit, tufano2019empirical}. To improve this set of models, Bahdanau \textit{et al.}~\cite{bahdanau} introduced attention mechanism where the decoder can focus or `attend to' the most important parts of the input sequence. The capabilities of sequence-to-sequence model are proven in summarization \cite{see2017get}, question answering \cite{seq2seqSquad}, Named Entity Recognition \cite{ner-seq2seq}, and many other tasks in natural language processing.  

%Seq2seq models originated for Neural Machine Translation (NMT), where a sentence from one language is translated to the sentence in another language. 
%Since then, its capabilities are proven in summarization \cite{see2017get}, question answering \cite{seq2seqSquad}, Named Entity Recognition \cite{ner-seq2seq}, and many other tasks in Natural Language Processing. 

%\textbf{Attention Mechanism:} Basic RNN, such as LSTM~\cite{hochreiter1997long} tends to perform poorly on long input sequence because of long-range dependency problem. To overcome this problem, Bahdanau \textit{\textit{et al.}} proposed Attention Mechanism~\cite{bahdanau}. Attention mechanism stores all the intermediate hidden states of a seq2seq encoder as a context vector, so that while generating a sequnece, the decoder can focus or `attend to' the most important parts of the input sequence. 
%Attention mechanism significantly improved the capacity of seq2seq models by enabling them to remember long-range dependencies in input tokens. Programming language tokens usually has a long range dependency, for example, there can be an arbitrary number of lines between a variable declaration and calling. Attention mechanism helps keep track of these type of long-distance dependencies.

\textbf{Copy Mechanism:} Basic seq2seq networks work on a fixed vocabulary for input and output sequence and consequently fails to account for any token outside the vocabulary. Copy mechanism allows seq2seq models to overcome this Out-of-Vocabulary (OOV) problem. Programming languages generally result in a large vocabulary. In previous studies \cite{chen2018sequencer,codit}, copy mechanism \cite{copy} has already been proven effective for this \textit{large vocab problem}~\cite{infinitevar}. When the seq2seq decoder faces an OOV token, the copy mechanism enables the decoder to copy the token directly from the input token stream and place it to the output token stream.

%instead of blindly discarding it. This allows our model to copy a token from the review comment and apply it to the fix. It is also effective in propagating input code tokens to output, because except from a few buggy tokens, most tokens remain unchanged in program repair.

\textbf{Defect \& Repair:} In software engineering, a defect is a deviation from the requirements \cite{defect}. A defect is not necessarily a bug that represents a coding error. It can be an explicit requirement, such as a program functionality or passing test suite, or it can be an implicit requirement such as avoiding spelling mistakes, following a naming convention or maintaining a consistent coding style. \toufique{Does other paper (speially [40]) call this implicit requirements as defect? If not try to avoid this kind of line} On the contrary, program repair is commonly associated with bug-fixing. In this study, we consider program repair in a broader sense of resolving defects. Code reviews help developers to identify and resolve these defects quickly and efficiently. We define program repair as the act of making appropriate changes to source code in response to a code review so that the defect no longer exists in the source code.

%A common source of defects is gap with the requirement, e.g., unrecognized requirements that result in errors of omission by the program designer \cite{defect-book}. The requirements can be non-functional/technical ones such as testability, scalability, maintainability, usability, performance, and security. Code reviews help developers to identify and resolve these defects quickly and efficiently.

%\textbf{Repair:} 


%no need ... too trivial
%\textbf{Developer:} Throughout this paper, `developer' is regarded as the person who is responsible for fixing the source code once a review comment is submitted. The developer may or may not be the author of the original source code file, or the commit.

